Low-Subpacketization MIMO Coded Caching with Flexible Stream Allocation

Subpacketization remains a major obstacle to the practical deployment of coded caching (CC) in multi-antenna wireless networks. In this paper, we propose a low-complexity multiple-input multiple-output (MIMO) CC scheme that enables flexible delivery rate adaptation while substantially reducing subpacketization requirements. The proposed design employs a virtual broadcast-channel decomposition to align cache-profile placement with flexible MIMO stream elevation which extends the shared-cache model to multi-antenna receivers. This enables flexible selection of feasible user and stream configurations, thereby providing explicit control over the spatial multiplexing gain under linear decodability constraints. Analytical results show that the proposed framework can asymptotically approach the best-known achievable degrees of freedom (DoF) under linear decodability constraints while requiring orders-of-magnitude lower subpacketization than existing schemes. Numerical evaluations further demonstrate that this flexibility yields notable throughput improvements at practical signal-to-noise ratios.

==> Figs/Symmetric_rate_Prop_SOTA_Comparison.tex <==
SNR		SCMIMOCComg18beta2				SCMIMOCComg18beta1			SCMIMOCComg14beta2				SCMIMOCComg15beta2					SCMIMOCComg16beta2				SCMIMOCComg24beta1				MUMIMOomg13beta1		
																												
0		29.3038035435469				29.2451542894323			30.1192289981295					30.489				29.6945776974030				27.8908751356576				21.7480446509832		
5		61.2370863474696				60.7453562167442			65.5131965930521					64.863				63.0381827623292				56.4263551196575				40.2715222199375		
10		108.909305957138				106.224074773682			123.762507543023					120.642				115.917899570185				100.600139291910				67.2875112376774		
15		169.413840595215				160.343779053781			200.773337537158					196.776				188.830578390729				161.576637142359				102.647818254632		
20		240.095356653109				218.181624970917			287.819832817299					286.614				278.721038761498				233.684960497903				142.797119454906		
25		321.021846452742				277.315333661041			378.830685557212					381.363				378.743362113604				310.719045371798				184.872703091928		
30		418.963827210563				336.925208055810			471.153940739457					481.299				482.876800000000				387.8544				228.211708870361		


==> Figs/sig_Theta_max_1e4.tex <==
K		MIMOCC	SCMIMOCC		MIMOCCWSA
					
20		18	24		24
40		18	36		32
60		18	45		32
80		18	48		32
100		18	48		32
120		18	48		32
140		18	48		32
160		18	48		32
180		18	48		32
200		18	48		32
220		18	48		32


==> Figs/sig_Theta_max_1e6.tex <==
K		MIMOCCWSA			MIMOCC		SCMIMOCC
							
20		24			30		24
40		32			30		36
60		32			30		48
80		32			30		60
100		32			30		63.83
120		32			30		75
140		32			30		75
160		32			30		75
180		32			30		75
200		32			30		75
220		32			30		75


==> Figs/sig_Theta_max_3e3.tex <==
K		MIMOCCWSA			MIMOCC		SCMIMOCC			MUMIMO
										
										
20		24			12		20.966			13
40		24			12		20.966			13
60		28			12		25.333			13
80		32			12		32			13
100		32			12		34.809			13
120		32			12		38.266			13
140		32			12		42.56			13
160		32			12		48			13
180		32			12		48			13
200		32			12		 48			13
220		32			12		48			13


==> Figs/uncosntrained_MIMO_CC_L16_G6_gamma_0.1.tex <==
K		MIMOCC		SCMIMOCC
				
20		30		24
40		42		36
60		54		48
80		66		60
100		78		72
120		90		84
140		102		96
160		114		108
180		126		120
200		138		132
220		150		144

